A Practical Recipe for Federated Learning Under Statistical Heterogeneity Experimental Design

Federated Learning (FL) has been an area of active research in recent years. There have been numerous studies in FL to make it more successful in the presence of data heterogeneity. However, despite the existence of many publications, the state of progress in the field is unknown. Many of the works use inconsistent experimental settings and there are no comprehensive studies on the effect of FL-specific experimental variables on the results and practical insights for a more comparable and consistent FL experimental setup. Furthermore, the existence of several benchmarks and confounding variables has further complicated the issue of inconsistency and ambiguity. In this work, we present the first comprehensive study on the effect of FL-specific experimental variables in relation to each other and performance results, bringing several insights and recommendations for designing a meaningful and well-incentivized FL experimental setup. We further aid the community by releasing FedZoo-Bench, an open-source library based on PyTorch with pre-implementation of 22 state-of-the-art methods, and a broad set of standardized and customizable features available at https://github.com/MMorafah/FedZoo-Bench. We also provide a comprehensive comparison of several state-of-the-art (SOTA) methods to better understand the current state of the field and existing limitations.

==> Literature-Analysis.tex <==
\section{Findings From The Literature}
In this section we provide our findings from the literature after reviewing a corpus of 200 papers. 
\subsection{Overview of Our Corpus}

\subsection{Non-IID Partitioning}
In the existing literature, the majority of works have focused on label distribution skew case. We find the following ways to simulate label distribution skew from the prior arts: 
\begin{itemize}
    \item \textbf{Label skew($p\%$):} in this case $p\%$ of the total classes are being randomly selected for each clients; then, each class data points are being partitioned amongst the clients who have that class.
    \item \textbf{Label Dir($\alpha$):} in this case each client draws a random vector from $\textit{Dir}(\alpha)$ for their class data points; then, each class data points are being partitioned amongst clients based on each clients' proportions.
    \item \textbf{Random shard($p$):} in this case, dataset is being partitioned into shards based on the number of clients, where each shard has only one class; then, each client receives $p$ random shards. In this scenario, clients have at most $p$ classes. 
    \item \textbf{Quantity Dir($\alpha$):} in this case each client draws a random number from $\textit{Dir}(\alpha)$ for their data points; then, data points are being randomly partitioned amongst clients based on each clients' data proportions.
    \item \textbf{Affine Distribution Shift:}
    \item \textbf{Feature noise:} 
\end{itemize}
Figure~\ref{} shows the demographic percentage of Non-IID simulation ways used in our corpus. Leaf also provides a simulated Non-IID partitions based the natural inherent Non-IID.

\subsection{Motivation for Personalization}

\subsection{Evaluation Metrics}

\subsection{Confounding Variables}

\subsection{Differences in Methodology}

\subsection{Hyper-parameters and Settings}
In fact we find that prior works compare with each other under different settings and hyper-parameters. Figure~\ref{} shows 
\begin{itemize}
    \item Dataset and Architecture demographic
    \item Accuracy results demographic 
    \item Non-IID setting demographic
\end{itemize}


==> algorithms.tex <==
\section{Algorithms}


\begin{algorithm}[H]
\caption{Federated Learning}
\label{alg:FedAvg}

% \DontPrintSemicolon
% \SetCommentSty{mycommfont}
% \SetAlgoLined
% \SetKwInOut{Req}{Require}
% \SetKwFunction{FClient}{ClientUpdate}
% \SetKwProg{Fn}{}{:}{}

\begin{algorithmic}[1]
\REQUIRE number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$).
%\SetKwProg{Fn}{Server Executes}{:}{}
\STATE \textbf{Server Executes:}
\STATE Initialize the server model with $\btheta_g^0$ \;
\FOR {each round $t = 0, 1, \ldots, T-1$}
\STATE $m \leftarrow {\rm{max}}(C \cdot N,1)$ \;
\STATE $S_t \leftarrow $(random set of m clients) \; %\tcp*{set of $m$ available clients}
\FOR {each client $k \in S_t$ \rm{\textbf{in parallel}}}
\STATE $\btheta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \btheta^t_{g} )$ \; 
%$\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
\ENDFOR
\STATE $\btheta^{t+1}_{g}=\mathtt{ModelFusion}(\{\btheta_k \}_{k \in S_t})$
\ENDFOR
\vspace{1mm}
\FUNCTION {$\mathtt{ClientUpdate}(k, \btheta^t_{g})$}
\STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
\STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k^{train}$ into batches of Size $B$})\;
\FOR {each local epoch $ \in \{1, \ldots, E\}$}
\FOR {each batch $\mathbf{b} \in \mathcal{B}$}
\STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} \ell(f_k(\bx; \btheta^{t}_k), y)$\;
\ENDFOR
\ENDFOR
\STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
\ENDFUNCTION
% \Fn{\FClient{$k, \btheta^t_{g}$}}{
%     \STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
%     \STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
%     \For {each local epoch $i = 1, \dots, E$} {
%         \For {each batch $\mathbf{b} \in \mathcal{B}$} {
%             \STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} f_k(\btheta^{t}_k; \mathbf{b})$\;
%         }
%     }
%     \STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
%     \KwRet $\btheta^{t+1}_{k}$\;
% }
\end{algorithmic}
\end{algorithm}


% \begin{algorithm}[H]
% \caption{FedAvg}
% \label{alg:FedAvg}

% % \DontPrintSemicolon
% % \SetCommentSty{mycommfont}
% % \SetAlgoLined
% % \SetKwInOut{Req}{Require}
% % \SetKwFunction{FClient}{ClientUpdate}
% % \SetKwProg{Fn}{}{:}{}

% \begin{algorithmic}[1]
% \STATE \textbf{Require:} number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$).
% %\SetKwProg{Fn}{Server Executes}{:}{}
% \STATE \textbf{Server Executes:}
% \STATE $\quad$ Initialize the server model with $\btheta_g^0$ \;
% \FOR {each round $t = 0, 1, \dots, T-1$}
% \STATE $\quad$ $m \leftarrow {\rm{max}}(C \cdot N,1)$ \;
% \STATE $\quad$ $S_t \leftarrow $(random set of m clients) \; %\tcp*{set of $m$ available clients}
% $\quad$ \FOR {each client $k \in S_t$ \rm{\textbf{in parallel}}}
% \STATE $\quad$ $\btheta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \btheta^t_{g} )$ \; 
% %$\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
% \ENDFOR
% \STATE $\quad$ $\btheta^{t+1}_{g}=\mathtt{ModelFusion}(\{\btheta_k \}_{k \in S_t})$
% \ENDFOR
% \vspace{1mm}
% \FUNCTION {$\mathtt{ClientUpdate}(k, \btheta^t_{g})$}
% \STATE H
% \ENDFUNCTION
% % \Fn{\FClient{$k, \btheta^t_{g}$}}{
% %     \STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
% %     \STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
% %     \For {each local epoch $i = 1, \dots, E$} {
% %         \For {each batch $\mathbf{b} \in \mathcal{B}$} {
% %             \STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} f_k(\btheta^{t}_k; \mathbf{b})$\;
% %         }
% %     }
% %     \STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
% %     \KwRet $\btheta^{t+1}_{k}$\;
% % }
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% \caption{FedProx}
% \label{alg:FedProx}

% \DontPrintSemicolon
% \SetCommentSty{mycommfont}
% \SetAlgoLined
% \SetKwInOut{Req}{Require}
% \SetKwFunction{FClient}{ClientUpdate}

% \Req{number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), 
% local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$), FedProx parameter ($\mu$)\;}
% \SetKwProg{Fn}{Server Executes}{:}{}
% \Fn{}{
% Initialize the server model with $\theta_g^0$ \;
% \For {each round $t = 0, 1, \dots, T-1$} {
%  $m \leftarrow {\rm{max}}(C \cdot N,1)$\;
%  $S_t \leftarrow $(random set of m clients)\; %\tcp*{set of $m$ available clients}
% \For  {each client $k \in S_t$ \rm{\textbf{in parallel}}}
% { 
% $\theta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \theta^t_{g} )$ \; 
% }

% $\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
% }
% }
% %\Indm
% \SetKwProg{Fn}{}{:}{}
% \Fn{\FClient{$k, \theta^t_{g}$}}{
%      $\theta^{t}_k \leftarrow \theta^t_{g}$\;
%      $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
%     \For {each local epoch $i = 1, \dots, E$} {
%         \For {each batch $\mathbf{b} \in \mathcal{B}$} 
%         {
%              $\theta^{t+1}_k \leftarrow \argmin_{\theta_k} \mathbb{E} \left[ f(\theta_k; \mathbf{b}) \right] + \frac{\mu}{2} ||\theta_k - \theta^t_k||^2$\;
%         }
%     }
%     $\theta^{t+1}_k \leftarrow \theta^{t}_k$\;
%     \KwRet $\theta^{t+1}_{k}$\;
% }
% \end{algorithm}



==> organization.tex <==
\begin{enumerate}
    \item a meta-analysis on the literature
    \item Inconsistency in the literature (accuracy, comparison, different artificial settings)
    \item Provide a thorough evaluation metrics
    \item Re-implementation of many algorithms and release FedZoo benchmark
    \item Effectively compare different FL algorithms under settings and rank them 
    \item Design and Propose experimental suggestions for the community
\end{enumerate}

\begin{itemize}
    \item when to personalize? (different niid, epoch, alg)
    \item accuracy metrics (test sample, train sample) only for fedavg. (different niid)
    \item gain with more communication rounds? (different niid, all alg)
    \item gain with more local epochs? (different niid, algs)
    \item scailability (algs)
    \item generalization to new commers (algs) 
    \item Fairness? (algs)
    \item designing federated experimental settings
\end{itemize}


%  In Karimireddy et al. (2019), authors argue that if
% these hyperparameters are not carefully tuned, it will result in the divergence of FedAvg, as local models may drift
% significantly from each other. Therefore, in the presence of statistical data heterogeneity, the global model might
% not generalize well on the local data of each client individually (Jiang et al., 2019). This is even more crucial in
% fairness-critical systems such as medical diagnosis (Li and Wang, 2019), where poor performance on local clients
% could result in damaging consequences.
